QM/MM Methods for Crystalline Defects. Part 3: Machine-Learned Interatomic Potentials

We develop and analyze a framework for consistent QM/MM (quantum/classic) hybrid models of crystalline defects, which admits general atomistic interactions including traditional off-the-shell interatomic potentials as well as state of art "machine-learned interatomic potentials". We (i) establish an a priori error estimate for the QM/MM approximations in terms of matching conditions between the MM and QM models, and (ii) demonstrate how to use these matching conditions to construct practical machine learned MM potentials specifically for QM/MM simulations.

==> old versions/qmmmV1.tex <==
% qmmm

\section{QM/MM coupling for crystalline defects}
\label{sec:qmmm}
\setcounter{equation}{0}

QM/MM coupling schemes can be in general categorized in the light of whether they link the QM and MM regions on the level of energies or forces: the energy-based methods construct a hybrid total energy functional and seek the local minimizer of the functional, while the force-based methods solve the force balance equation with QM and MM contributions.  In this section, we will provide error estimates for both of the coupling schemes.

% Depending on how QM model and MM model are coupled, QM/MM coupling methods can be broadly classified as either force or energy-based \cite{chen17}. Energy-based couplings define a hybrid energy functional as a combination of atomistic and continuum energy functionals, and this hybrid energy functional is then minimized over a class of admissible deformations. Force-based couplings instead derive quantum and molecular forces from the separate energies and then equilibrate them.



\subsection{Decomposition of the configuration}
\label{sec:decomposition}

We decompose the reference configuration $\L$ into three disjoint sets, $\L = \LQM\cup \LMM\cup \LFF$, where $\LQM$ denotes the QM region, which contains the defect core $B_{R_{\rm DEF}}$, $\LMM$ denotes the MM region, and $\LFF$ denotes the far-field region where atom positions will be frozen on the basis of the far-field predictor. Moreover, for the purpose of eliminating spurious interface effects, we define a buffer region $\Lbuf\subset\LMM$ surrounding $\LQM$ such that all atoms in $\Lbuf\cup\LQM$ are involved in the evaluation of the site energies in $\LQM$. For simple cases, we can use balls centred at the defect core to decompose $\Lambda$, and use parameters $\RQM$, $\RMM$ and $\Rbuf$ to represent the respective radii (see Figure \ref{fig:decomposition} for a schematic plot of the partition).

\begin{figure}[!htb]
        \centering
        \includegraphics[height=6.0cm]{figs/decomposition.pdf}
        \caption{Domain decomposition in the QM/MM coupling scheme.}
        \label{fig:decomposition}
\end{figure}

Given a specific domain decomposition, we propose the general idea of the energy-based methods used in this paper, which mix the site energies computed by QM and MM methods in their respective regions,
\begin{eqnarray}\label{energy-local}
E(u) =
\sum_{\ell\in \LQM}V_{\ell}^{\rm QM}(Du(\ell))
+ \sum_{\ell\in \LMM}V_{\ell}^{\rm MM}(Du(\ell))
\end{eqnarray}
with $\VQM_{\ell}, \VMM_{\ell}$ denoting the site potential associated to the $\ell$-th atomic site with QM and MM methods in the corresponding region respectively. The advantage of energy-based methods is that they are naturally energy conserving while the shortcoming is the spurious interface effects might be significant between the QM and MM regions. To mitigate such effects, we define the buffer layers surrounding the QM and MM regions, so that each atom can see their neighbour as much as possible.

The force-based methods, which combine QM
forces of atoms in the QM region with MM forces of atoms in the MM region, can be defined as
\begin{eqnarray}\label{eq:Fidea}
  \F_{\ell}(u) = \left\{\begin{array}{ll}
\F^{\rm QM}_{\ell}(u) & {\rm if}~\ell\in \LQM \\[1ex]
\F^{\rm MM}_{\ell}(u) & {\rm if}~\ell\in \LMM
\end{array}\right..
\end{eqnarray}
The force-based methods achieve no spurious interface forces at the expense of a non-conservative force field, which means it can not be given by the Euler-Lagrange equation for a certain energy. 

\subsection{MM models}
\label{sec:MMmodels}

% \chc{maybe this is a good point to discuss different interatomic potentials or force fields, and how important it is in QM/MM coupling...}

% briefly introduction
In this section, we mainly discuss the choice of MM model, which remains to be considerable since it will have crucial influence in our error estimates. 
%We note in advance that our analysis can still be applied to general MM potentials.

% classical 
Like in other commonly used QM/MM schemes, first simple choice of MM potential $\VMM: (\R^d)^{\LhomS} \rightarrow \R$ is the classical interatomic potential such as EAM (Embedded Atom Method) potential \cite{Daw1984a} and Finnis-Sinclair model \cite{finnis03}. However, it is pointed out in \cite{bernstein09} that matching the first derivatives of the force or the second order derivatives of the energy can guarantee that spurious forces are eliminated for near equilibrium configurations. Hence, the MM model should be tuned to interact “correctly” with the QM model instead of using “black-box” MM potentials. We will also show the inconsistency of using the classical potentials as a special case in the framework of this paper in Remark \ref{re:example}.

% QMMM2
In previous work of this series \cite{chen17}, we construct the MM model as an explicit and controllable approximation of the QM model because of the strong locality studied in \cite{chen16}, which is reminiscent of the force matching technique \cite{bernstein09}, but the key difference is in \cite{chen17} we match the site energies rather than total energies. We build the idealized MM potential $\VMM: (\R^d)^{\LhomS} \rightarrow \R$ by $k$-th order Taylor expansion of $\Vhom$ about the far-field lattice state,
\begin{eqnarray}\label{eq:taylor_E}
\VMM\big({\bm g}\big) := T_k\Vhom\big({\bm g}\big) 
:= \Vhom({\bf 0}) + \sum_{j=1}^k \frac{1}{j!} \delta^j \Vhom({\bf 0})\left[{\bm g}^{\otimes j}\right]
\quad{\rm with}~~k\geq 2,
\end{eqnarray}
which matches the QM model exactly. Meanwhile, we also denote the $k$-th order Taylor expansion of $\F^{\rm h}$ for force-mixing methods
\begin{eqnarray}\label{eq:taylor_F}
\FMM\big({\bm g}\big) := T_k\F^{\rm h}\big({\bm g}\big) 
:= \sum_{j=1}^k \frac{1}{j!} \delta^j \F^{\rm h}({\bf 0})\left[{\bm g}^{\otimes j}\right]
\quad{\rm with}~~k\geq 1.
\end{eqnarray}
However, we mention that the computational cost for higher-order Taylor expansions is severe for the case of slowly decaying elastic fields (dislocations, cracks) and it is not suitable for multi-lattice. So it remains to be explored whether MM site energies via Taylor expansions could be replaced with alternative approximations. 

In this paper, we mainly focus on the data-driven interatomic potentials as the MM potential $\VMM: (\R^d)^{\LhomS} \rightarrow \R$, which are based on spherical harmonic and are trained by the data from QM potential $\Vhom$ so that they can fit the QM model well in the QM/MM coupling. In contrast to kernel based and artificial neural network models, the explicit decomposition of the total energy as a sum of atomic body-ordered terms allows to keep the dimensionality of the fit reasonably low. 

% cutoff, locality and regularity of MM
Similar to the definition of the regularity of $V_{\ell}$ by \asSER, for the general MM potential $\VMM$, we denote the partial derivatives by 
\begin{eqnarray}\label{eq:dVMM}
\VMM_{,{\bm \rho}}\big({\bm g}\big) :=
\frac{\partial^j \VMM \big({\bm g}\big)}
{\partial {\bm g}_{\rho_1}\cdots\partial{\bm g}_{\rho_j}}
\qquad{\rm for}\quad{\bm g}\in(\R^d)^{\LhomS}.
\end{eqnarray}
We also denote the partial derivatives of MM forces $\F^{\rm MM}$ as 
\begin{eqnarray}\label{eq:dFMM}
    \F^{\rm MM}_{, {\pmb \ell}} (w) := \frac{\partial^j \F^{\rm MM}(w)}  {\partial w_{\ell_1}\cdots\partial w_{\ell_j}}
    \qquad{\rm for}\quad w:\Lhom\rightarrow \R^d \quad{\rm and}\quad \pmb{\ell}=(\ell_1\cdots,\ell_j)\in(\Lhom)^j.
\end{eqnarray}
We assume that the general MM potential $\VMM$ should also satisfies the conditions \asSEL, \asSEH. It is worth mentioning that the cutoff of the interaction range of the MM potential plays an important role in constructing the  data-driven interatomic potential. Analytically we will put it into the training error defined in the following see also Remark \ref{re:cutoff} for more details.

Recalling that $\Vhom:(\R^d)^{\LhomS}\rightarrow\R$ is denoted as the homogeneous site potential, we now define the training error for energy-mixing scheme $\efit_j$ for $j=1,...,K$:
\begin{align}\label{training_error}
\efit_j &:= \big|\delta^{j} V^{\rm h}_{,\pmb \rho} - \delta^{j} \VMM_{,\pmb \rho}\big|_{w^{-1}} \nonumber \\
&:= \left(\sum_{\pmb\rho = (\rho_1, ..., \rho_j)\in (\LhomS)^j}\Big|V^{\rm h}_{,\pmb\rho}(\pmb 0) - \VMM_{,\pmb\rho}(\pmb 0)\Big|^2 \mathbf{W}_j^{-1}(\pmb\rho) \right)^{1/2},
% \Big(\prod^{j}_{i=1} w(|\rho_i|)\Big)^{-1}  \right)^{1/2},
\end{align}
where $V^{\rm h}_{,\pmb\rho}(\pmb 0)$ and $\VMM_{,\pmb\rho}(\pmb 0)$ are defined by \eqref{eq:dV} and \eqref{eq:dVMM} respectively, $\Wb_j:(\LhomS)^j \rightarrow \R$ is the weight function which is related to the form in assumption \asSEL \quad and will be determined specifically in numerical simulations in Section \ref{sec:SHIPs}. \ysc{2: In our current analysis, we need $\Wb^{-1}_j$ to appear in the definition of $\efit_j$, so that the norm $\|Dv\|_{\ell^2_{w}}$ can be extracted out. Please see \eqref{eq:T51} for details. But the weight $\Wb^{-1}_j$ seems to be a little bit wired, which means that the weight gets larger when $|\rho|$ gets larger?}
% \chc{the weight here is more complicated, which is related to the form in assumption \asSEL, and could also involve $w_j$? please check...}
We do not define $\efit_0$ since the constant will not influence the equilibrium state.

In the meantime, we define the training error for force-mixing scheme $\ffit_j$ for $j=1, ..., K-1$:
\begin{align}\label{training_error_F}
\ffit_j &:= \big|\F^{\rm h}_{,\pmb \ell} - \FMM_{,\pmb \ell} \big|_{w^{-1}} \nonumber \\
&:= \left(\sum_{\pmb\ell = (\ell_1, ..., \ell_j)\in (\Lhom)^j}\Big|\F^{\rm h}_{,\pmb\ell}(\pmb{0}) - \FMM_{,\pmb\ell}(\pmb{0})\Big|^2\mathbf{W}_j^{-1}(\pmb\ell) \right)^{1/2},
% \Big(\prod^{j}_{i=1}w(|\ell_i|)\Big)^{-1} \right)^{1/2},
\end{align}
where $\mathcal{F}^{\rm h}_{,\pmb \ell}(\pmb{0})$ and $\mathcal{F}^{\rm MM}_{,\pmb \ell}(\pmb{0})$ are defined by \eqref{eq:dF} and \eqref{eq:dFMM} respectively, and $\mathbf{W}_j: (\Lhom)^j \rightarrow \R$ is the weight function. We remark that $\ffit_0$ is not needed since the reference lattice is an equilibrium.


% \chc{mention the old ideas of construction, idea of force matching, idea of Taylor expansion ... also the data-driven kernel based and artificial neural network models ... see Remark 2.1 in \cite{chen17}}



\subsection{Energy mixing}
\label{sec:energyMix}

%\chc{please check the whole proof carefully, although no essential difference, but the formulation of the locality \asSEL, the stability \asLS, and the decay result \eqref{eq:ubar-decay} are all in a different way ...}

% \chc{should clarify the difference between $\VQM_{\ell}$ and $V_{\ell}$ at this point ...}
For the purpose of introducing the coupling schemes, we denote the site potential in a given subsystems $\Omega \subset \L$ by $V^{\Omega}_{\ell}({\pmb g})$, which means the interactions only occur in $\Omega$. The site potential in QM region $B_{\RQM}$ is then denoted as 
\begin{eqnarray}\label{eq:vqm}
\VQM_{\ell}({\pmb g}) := V^{\Lbuf\cup\LQM}_{\ell}({\pmb g}).
\end{eqnarray}
% \cys{Discuss: should have a better way to describe, or will have $\Rbuf$ in the error estimates.}

% interpolation
To map the displacements from a defective reference configuration $\L$ to the corresponding homogeneous lattice $\Lhom$, following \cite[Lemma D.1]{chen19}, we can construct an interpolation operator $I^{\rm h}_1: \UsH(\L) \rightarrow \UsH(\Lhom)$ satisfying for $C_{*}>0$
\begin{eqnarray}\label{eq:eqI}
\|DI^{\rm h}_1u\|_{\ell^2_{\mathcal{N}}(\Lhom)}\leq C_{*}\|Du\|_{\ell^2_{\mathcal{N}}(\L)}, \quad \forall u \in \UsH(\L).
\end{eqnarray}

If we approximate the site potential $\Vhom(Du(\ell))$ by some MM site potential $\VMM: (\R^d)^{\LhomS} \rightarrow \R$ briefly introduced in Section \ref{sec:MMmodels}, and we also require the smoothness of $\VMM$ say that $\VMM \in C^{K}$ for $K \in \N$, following the general ideas of QM/MM coupling schemes given in Section \ref{sec:decomposition}, then the QM/MM hybrid energy difference functional can be specified as 
\begin{align}\label{eq:hybrid_mid_energy}
\EH(u)  := \sum_{\ell\in \LQM} \Big( \VQM_{\ell}\big(D u(\ell)\big)  - \VQM_{\ell}\big(\pmb{0}\big) \Big)
+ \sum_{\ell\in \LMM\cup\LFF}  \Big( \VMM\big(D I^{\rm h}_{1}u(\ell)\big) - \VMM\big(\pmb{0}\big) \Big), 
\end{align}
where the interpolation operator $I^{\rm h}_{1}: \UsH(\L) \rightarrow \UsH(\Lhom)$ is constructed above.
\ysc{1: The stencil for $\VMM$ is now over the whole lattice, which include the case of finite range interaction.
The parameter $R_{\rm CUT}$ is not needed, whose truncation error now goes into $\efit_j$ defined by \eqref{training_error}. Does this sounds okay for you?} 

We note that \eqref{eq:hybrid_mid_energy} is the generalization of that in \cite{chen17}. However, ``the spurious forces" may happen in this case, which will cause the inconsistency in the error estimates, see \eqref{eq:T52_nogfc} for details. Hence, we require the examination of such forces so that we can know when and how they can be removed.

% patch test and ghost force correction.
In order to construct consistent hybrid energy functional, like used in the design of consistent atomistic-to-continuum coupling methods (e.g. \cite{Chen12ghost, mlco2013, colz2012}), we need to enforce the so-called patch tests \cite{co2011} for the energy functional  $\EH(u)$, namely, energy patch test and force patch test.
The patch test is often employed in the theory of finite element methods \cite{Belytschko00, strang08} as a simple test for consistency.

\begin{flushleft}\label{as:patch}
{\it Patch test:} ~
An energy functional $\EH(u)$ is patch test consistent if 
for $V_{\ell} \equiv \Vhom$, $\L = \Lhom$, 
it satisfies $\EH(\pmb{0})=\mathcal{E}(\pmb{0})$ and $\<\delta\EH(\pmb{0}), v\>=0$, for all $v \in \UsH(\L)$.
\end{flushleft}

From the definition above, we observe that whether $\EH(u)$ defined by \eqref{eq:hybrid_mid_energy} is patch test consistent or not highly depends on the choices of $\VMM$. As a matter of fact, $\EH(u)$ always has ``the spurious forces" (usually termed as {\it ghost forces}) near the interface if $\VMM$ is not chosen as the Taylor expansion of $\Vhom$ by \eqref{eq:taylor_E}. In order to remove the {\it ghost forces}, motivated by \cite{colz2016}, we combine the two popular practical schemes, ghost force correction and blending. We modify the total energy $\EH(u)$ by adding a blended correction term, that is,
\begin{eqnarray}\label{eq:hybrid_energy_BGFC}
\quad \Egfc(u) 
= \EH(u) - \<\delta\EH(\pmb{0}), \beta u\>, \qquad
\end{eqnarray}
where $\beta \in L^2(\R^d)$ is a blended function satisfying
\begin{eqnarray}\label{beta}
	\beta(x) =
	\left\{ \begin{array}{ll}
		0, & |x|<\RQM/2
		\\[1ex]
		1, & |x|>3\RQM/4  
	\end{array} \right. ,
\end{eqnarray}
with $\beta(x)$ a transition function from $0$ to $1$ such as affine function or sine function when $\RQM/2<|x|<3\RQM/4$. We mention that $b(x)\equiv1$ is suitable in our analysis.  
% and $|\nabla \beta| \leq 1/(4\RQM)$. \ysc{2: In our current analysis, we require $\beta$ to be smoothly varying, which is demonstrated in \eqref{eq:diff}. We can not prove the decay of consistency error when there is a sharp interface of $\beta$, (though I can achieve the convergence in numerics according to your suggestion)?} 

We are ready to define the QM/MM energy-mixing scheme without {\it ghost forces}
\begin{eqnarray}\label{eq:variational-problem-H}
\bar u^{\rm H} \in \arg\min \big\{ \mathcal{E}^{\rm GFC}(u), u \in \Admu^{\rm H}(\L) \big\}, 
\end{eqnarray}
where the admissible set is defined by
\begin{eqnarray*}
\Admu^{\rm H}(\L):= \big\{ u\in\Usx(\L) ~:~ x_0+u\in\Adm_0(\L) \big\}
\end{eqnarray*}
with
\begin{eqnarray}\label{e-mix-space}
\Usx(\L) := \left\{ u \in \Us^{1,2}(\L)  ~\lvert~ u=0~{\rm in}~\Lambda^{\rm FF} \right\}.
\end{eqnarray}

The QM/MM energy mixing scheme \eqref{eq:variational-problem-H} satisfies the following approximation error estimate. For the sake of simplicity, the proof are given in the appendix.

\begin{theorem}
	Let $\bar{u}$ and $\uH$ be the solutions of \eqref{eq:variational-problem} and \eqref{eq:variational-problem-H}, respectively. If the assumptions \asSEL, \asSER, \asSEH ~are satisfied, $\RQM$ is sufficiently large, and the training errors $\efit_j, j=1,...,K$ defined by \eqref{training_error} are sufficiently small, then there exists constants $C$ and $\kappa$ that does not depend on $\RQM, \RMM, \efit_j$ such that
	\begin{eqnarray}\label{res-bound}
	\|D\bar{u}-D\uH\|_{\ell^2_{\mathcal{N}}} \leq C\left(\sum^{K}_{j=2} \efit_j  R^{-\alpha_j}_{\rm QM} +  R^{-\alpha_{K+1}}_{\rm QM} + R^{-d/2}_{\rm MM} + e^{-\kappa \Rbuf} + e^{-\kappa \RQM}\right),
	\end{eqnarray}
	where $\alpha_j = (2j-3)d/2$.
\end{theorem}

\begin{remark}\label{re:example}
We present two examples to demonstrate how the training errors $\efit_j$ can influence the approximation error in \eqref{res-bound}. If MM potential $\VMM$ is chosen to be the $K$-th Taylor expansion of $\Vhom$ by \eqref{eq:taylor_E}, then $\efit_j$ vanish, for $j=1,...,K$. We can achieve the same error estimates as that in \cite[Theorem 4.1]{chen17}. If MM potential $\VMM$ is selected as a classical interatomic potential and can not match the QM model very well, which indicate the first two training errors $\efit_j, j=1,2$ are fixed to be relatively large, therefore according to \eqref{res-bound} the approximation error will not decay at all. In Section \ref{sec:simulations} we will numerically verify that for different levels of training error we can obtain different convergence rate.
% For $d=2$, if $k=2$, then $\|D\bar{u}-D\uH\|_{\ell^2_{\omega}} \lesssim \efit_2  R^{-1}_{\rm QM} + R^{-3}_{\rm QM} + R^{-1}_{\rm MM}$. If $k=3$, then $\|D\bar{u}-D\uH\|_{\ell^2_{\omega}} \lesssim \efit_2  R^{-1}_{\rm QM} + \efit_3  R^{-3}_{\rm QM} + R^{-5}_{\rm QM} + R^{-1}_{\rm MM}$.
\end{remark}

\begin{remark}\label{re:cutoff}
We remark that the cutoff of MM interaction range can affect the accuracy heavily in the error estimates \eqref{res-bound} via the training process. The reason why it does not appear in the right hand side of \eqref{res-bound} is that the errors coming from the cutoff of MM interaction range are already included in $\efit_{j}$ by way of choosing the weight function properly according to \eqref{training_error}.
% \cite{chen17} shows it decays exponentially with respect to $\Rbuf$. Hence, in this paper, we select $\Rbuf$ relatively large so that we can ignore its influence compared to other types of errors.
\end{remark}

\subsection{Force mixing}
\label{sec:forceMix}
To construct a force-based QM/MM coupling scheme, we follow the idea in Section \ref{sec:decomposition} by \eqref{eq:Fidea}. Similar the definition of $\VQM_{\ell}$ in the beginning of Section \ref{sec:energyMix}, we also denote the QM forces in QM region $B_{\RQM}$ as $\F^{\rm QM}_{\ell}$. 
We construct an approximation to the QM force on the homogeneous configuration $\F^{\rm h}$ by
$\FMM:(\R^d)^{\Lhom} \rightarrow \R$ in the spirit of that discussed in Section \ref{sec:MMmodels}.

We have the following force-mixing QM/MM coupling model:
\begin{eqnarray}\label{problem-f-mix}
	{\rm Find}~\uH\in \Admu^{\rm H}(\L), ~~ {\rm s.t.} \quad
	\F_{\ell}^{\rm H}\big(\bar{u}^{\rm H}\big) = 0
	\qquad \forall~\ell\in\LQM\cup\LMM
\end{eqnarray}
with the hybrid force
\begin{eqnarray}\label{F-H}
	\F_{\ell}^{\rm H}(u) =
	\left\{ \begin{array}{ll}
		\F^{\rm QM}_{\ell}(u) & \ell\in\LQM
		\\[1ex]
		\FMM\left( I_1^{\rm h}u(\cdot-\ell)
		 \right) & \ell\in\LMM  %\cup\LFF
	\end{array} \right. ,
\end{eqnarray}
where $I^{\rm h}_1: \UsH(\L) \rightarrow \UsH(\Lhom)$ is constructed in Section \ref{sec:energyMix}. \ysc{3: here no cutoff again.} We emphasize that $\FH$ is not a gradient of any energy functional.  For
$v:\L\rightarrow\R$, we will use the notation
$\big\<\FH(u),v\big\>:=\sum_{\ell\in\LQM\cup\LMM}\FH_{\ell}(u)\cdot v(\ell)$ in
our analysis.


\begin{theorem}
	Let $\bar{u}$ and $\uH$ be the solutions of \eqref{eq:problem-force} and \eqref{problem-f-mix}, respectively. If the assumptions \asSER, \asSEL, \asSEH~ are satisfied, $\RQM$ is sufficiently large and the training errors $\ffit_j$ defined by \eqref{training_error_F} are sufficiently small, then there exists a constant $C$ that does not depend on $\RQM, \RMM, \ffit_j$ such that
	\begin{eqnarray}\label{res-bound-F}
	\|D\bar{u}-D\uH\|_{\ell^2_{w}} \leq C\left(\sum^{K-1}_{j=1} \ffit_j  R^{-\alpha_j}_{\rm QM} + R^{-\alpha_{K}}_{\rm QM} + R^{-d/2}_{\rm MM}\right),
	\end{eqnarray}
	where the order $\alpha_j = (2j-1)d/2$.
\end{theorem}

% \ys{For $d=2$, if $k=1$, then $\|D\bar{u}-D\uH\|_{\ell^2_{\omega}} \lesssim \ffit_1  R^{-1}_{\rm QM} + R^{-3}_{\rm QM} + R^{-1}_{\rm MM}$. If $k=2$, then $\|D\bar{u}-D\uH\|_{\ell^2_{\omega}} \lesssim \ffit_1  R^{-1}_{\rm QM} + \ffit_2  R^{-3}_{\rm QM} + R^{-5}_{\rm QM} + R^{-1}_{\rm MM}$}



